Complexity of Safety and coSafety Fragments of Linear Temporal Logic

Linear Temporal Logic (LTL) is the de-facto standard temporal logic for system specification, whose foundational properties have been studied for over five decades. Safety and cosafety properties define notable fragments of LTL, where a prefix of a trace suffices to establish whether a formula is true or not over that trace. In this paper, we study the complexity of the problems of satisfiability, validity, and realizability over infinite and finite traces for the safety and cosafety fragments of LTL. As for satisfiability and validity over infinite traces, we prove that the majority of the fragments have the same complexity as full LTL, that is, they are PSPACE-complete. The picture is radically different for realizability: we find fragments with the same expressive power whose complexity varies from 2EXPTIME-complete (as full LTL) to EXPTIME-complete. Notably, for all cosafety fragments, the complexity of the three problems does not change passing from infinite to finite traces, while for all safety fragments the complexity of satisfiability (resp., realizability) over finite traces drops to NP-complete (resp., ${\Pi}^P_2$-complete).

==> sections/old.counter.tex <==
The methodology that we will use for proving hardness results is similar to
the one that we used for satisfiability, but applied to tiling games: for
cosafety (resp. safety) fragments we will use rectangle tiling games (resp.
infinite corridor tiling games). 
We will make the natural correspondence between Controller and Environment
players (of realizability) with Constructor and Saboteur players of tiling
games.
Finally, for proving the \EXPTIME[2]-hardness (resp. \EXPTIME-hardness), we
will use the variant with $n$ encoded in binary (resp. unary).

The hardness reductions of this section, as expected, is strongly based on
the encoding of tilings in temporal formulas, as described in the previous
section. However, there are four main problems that have to be addressed
when dealing with a reduction from tiling into realizability problems:
\begin{enumerate}
  \item the variables under the control of Environment and Controller
    players are disjoint while Saboteur and Constructor choose tiles from
    the same set $T$;
  \item a round between Environment and Controller creates a state of
    a trace (which, in our reduction, corresponds to a cell of a tiling),
    while a round between Saboteur and Constructor constists of two cells
    of a tiling;
  \item Environment moves before Controller, while Constructor moves before
    Saboteur (this point as well as the previous ones were already noted in
    \cite{cimatti2021extended});
  \item the encoding significantly changes depending on whether $n$ is
    encoded in unary (like in the previous section) or in binary.  The main
    cause of this difference are the constraints that involve timepoints at
    distance $n$ (like the horizontal constraint \hor, or \bcolumn,
    \sidetiling, \etc).  In the case $n$ is encoded in unary, using $n$
    nested \emph{tomorrow} or \emph{yesterday} is allowed, since the
    resulting formula will be of polynomial size with respect to the tiling
    problem.  On the contrary, if $n$ is encoded in binary, the formula
    used in the previous case is of exponential size and thus cannot be
    used in a reduction.
\end{enumerate}

In order to overcome these problems, we proceed as follows.  Given a tiling
structure $\tiling = \seq{ T, t_{\bor}, H, V}$, we will define a formula
$\phi_{n,\tiling}^{\game}$ such that:
\begin{enumerate*}[label=(\roman*)]
  \item its size is polynomial in the size of $\tiling$; and
  \item it is realizable iff Constructor has a strategy in the tiling game
    of $\tiling$.
\end{enumerate*}

We begin by describing the solution of the fourth problem, since it will
affect the description of the solution of the other points. The sequence of
$n$ nested temporal operators can be simulated by the use of a binary
counter, which requires only a logarithmic number of bits with respect to
$n$ and thus can be used as a valid alternative to $n$ nested temporal
operators, in the case $n$ is given in binary. For this purpose, we
introduce $m$ fresh proposition letters $c_0, \dots, c_{m-1}$ encoding
the bits of a binary counter modulo $n = 2^m$.

We will define $\phi_{n,\tiling}^{\game}$ over the alphabet $\Sigma
= \Uset\cup\Cset$, where $\Uset \coloneqq \set{t^u \mid t \in T}$ and
$\Cset \coloneqq \set{t^c \mid t \in T} \cup \set{c_0,\dots,c_{m-1}} \cup
\set{b}$. In the case in which $n$ is given in unary, we simply assume that
$m=0$ (\ie we do not use counter bits). This solves the first problem. Note
that the proposition letters $c_0,\dots,c_{n-1}$ as well as $b$ are set to
be \emph{controllable}: this because we want to ensure that, whenever the
formula is unrealizable, the reason is not a wrong marking of the top and
bottom border or a wrong increment of the counter but, rather, the
nonexistence of a strategy for Constructor for building a tiling.

For solving the second problem, we have to impose that, for any time point
$i$, Environment player plays at round $i$ iff Controller player plays at
round $i+1$ and they never play at the same round.  As for the third
problem, it suffices to force the formula $\firstplayer \coloneqq
\bigvee_{t\in T}t^u$ to be true at the initial time point.

In the following we define the formulas that we will use to address the
previous problems.  Let $\op$ be a unary temporal operator. 
\begin{itemize}
  \item \emph{Saboteur} plays at round $t$ iff \emph{Constructor} plays at
    round $t\pm 1$, and the two player never play in the same round:
    \begin{align*}
      \altern[\op] 
        &\coloneqq
        \bigvee_{t\in T} (t^u \iff \op(\bigvee_{t\in T} t^c)) \land
        \bigvee_{t\in T} (t^u \iff \bigwedge_{t\in T} \lnot t^c)
    \end{align*}
  \item At time point $t\pm 1$, the counter increments modulo $n$ with
    respect to time point $t$:
    \begin{align*}
      \counterinc[\op]
        &\coloneqq
          \bigwedge_{i=0}^{m-1} \counter[op][i]
    \end{align*}
    where:
    \begin{align*}
      \counter[\op][0]
        &\coloneqq
          \op(c_0) \iff \lnot c_0 \\
      \counter[\op][i]
        &\coloneqq
          \op(c_i) \iff ((\bigwedge_{j=0}^{i-1} c_j) \iff \lnot c_i)
    \end{align*}
  \item Let $i$ be a value between $0$ and $n-1$. We define the Boolean
    formula for checking whether the values of $c_0,\dots,c_{n-1}$
    represent the value $i$. Let $J_1 \subseteq \set{0,\dots,m-1}$ (resp.
    $J_2 \subseteq \set{0,\dots,m-1}$) be the set of positions with value
    $1$ (resp. $0$) in the binary representation of $i$.
    \begin{align*}
      \isnumber^i
        &\coloneqq
        \bigwedge_{j\in J_1} c_j \land \bigwedge_{j\in J_2} \lnot c_j
    \end{align*}
\end{itemize}


\begin{lemma}
\label{real:cosafetyltl}
  For realizability problem over infinite traces for \cosafetyltl is
  \EXPTIME[2]-complete.
\end{lemma}
\begin{proof}
  \emph{(Membership)}
  It follows from the \EXPTIME[2]-membership of \LTL realizability.

  \emph{(Hardness)}
  We reduce \textnormal{EXP-RECT-GAME} to the \cosafetyltl realizability.
  From now on, for each formula $\psi$ among \tile, \bcolumn[op],
  \bordertiling[op], \sidetiling[op], \hor[op], \ver[op], and
  \vertcolumn[op], let $\psi^\game$ be defined as $\psi[t \mapsto t^u \lor
  t^c]$.

  We begin by modifying all formulas that require $n$ nested temporal
  operators in such a way that they use the binary counter instead. 
  \begin{itemize}
    \item Version of $\bcolumn[X][\game]$ with the counter:
      \begin{align*}
        \overline{\bcolumn[X][\game]}
        \coloneqq
        (\isnumber^{0} \lor \isnumber^{n-1}) \iff b
      \end{align*}
    \item Version of $\sidetiling[X][\game]$ with the counter: we force
      $t_{\bor}$ to be true at all states before (and including) the first
      occurrence of a state in which the counter take value $n-1$.
      \begin{align*}
        \overline{\sidetiling[X][\game]}
        \coloneqq
        (t_{\bor} \land \lnot \isnumber^{n-1})\ltl{U}(t_{\bor} \land
        \isnumber^{n-1})
      \end{align*}
    \item Version of $\bordertiling[X][\game]$ with the counter:
      \begin{align*}
        \overline{\bordertiling[X][\game]}
        &\coloneqq
        ((\isnumber^{n-1} \lor \isnumber^0) \to b) \land  \\
        &\qquad
        ((\lnot \isnumber^{n-1} \land \lnot \isnumber^0) \to \lnot b) \land
        \\
        &\qquad
        (b \to t_{\bor})
      \end{align*}
    \item Version of $\hor[X][\game]$:
      \begin{align*}
        \overline{\hor[X][\game]}
        \coloneqq
      \end{align*}
    \item Version of $\vertcolumn[X][\game]$ with the counter:
      \begin{align*}
        \overline{\vertcolumn[X][\game]}
        \coloneqq
        (\bigvee_{(t,t') \in V} (t \land \ltl{X}
        t'))\ltl{U}(\isnumber^{n-1})
      \end{align*}
  \end{itemize}
  
  We define:
  \begin{align*}
    \init[X][\game]
      &\coloneqq 
      \bcolumn[X][\game] \land 
      \sidetiling[X][\game] \\
    \invariant[X][\game]
      &\coloneqq 
      \altern[X]
      \tile[][\game] \land 
      \bordertiling[X][\game] \land 
      \hor[X][\game] \land 
      \ver[X][\game] \\
    \goal[X][\game]
      &\coloneqq 
      \sidetiling[X][\game] \land 
      \vertcolumn[X][\game] \land
      \alterncolumn[X][\game]
  \end{align*}
  We set:
  \begin{align*}
    \phi_{n,\tiling}^{\game}
      \coloneqq
      \init[X][\game] \land (\invariant[X][\game] \ltl{U} \goal[X][\game])
  \end{align*}
  It holds that $\phi_{n,\tiling}^{\game}$ is of polynomial size with
  respect to the size of $\tiling$ and it is realizable iff Constructor has
  a winning strategy for \textnormal{EXP-RECT-GAME}.
\end{proof}


\begin{lemma}
\label{real:falpha}
  The realizability problem of $\ltl{F\alpha}$ is \EXPTIME-complete.
\end{lemma}
\begin{proof}
  \emph{(membership)} The crucial point is that $\alpha\in\LTLFP$ and we
  can build a \DFA for $\alpha$ with only a \emph{single} exponential
  blowup~\cite{de2021pure}(while in general formulas in \LTLf require two
  exponential blowups). Intuition: since \emph{``past already happened''},
  there is no need for nondeterminism. Once obtained the \DFA,
  a reachability game can be solved in linear time in the size of the
  arena~\cite{de2007concurrent}. Therefore, the overall complexity is
  \EXPTIME.

  Alternative proof of the membership: it derives from our journal paper
  FMSD.
  
  \emph{(hardness)} We consider the conditional planning problem with no
  trajectory constraints and a reachability goal. As described
  in~\cite{DeGiacomoV15,rintanen2004complexity}, this problem is
  \EXPTIME-complete. We reduce this problem into the satisfiability of
  $\ltl{F\alpha}$.
\end{proof}

\begin{lemma}
\label{real:galpha}
  The realizability problem of $\ltl{G\alpha}$ is \EXPTIME-complete.
\end{lemma}
\begin{proof}
  \emph{(membership)} It follows directly from the fact that
  $\ltl{G(\alpha)}$ is a syntactical fragment of \LTLEBRP with no bounded
  operators, and the realizability problem of this latter fragment is
  \EXPTIME-complete.

  \emph{(hardess)} Rectangle Tiling games with $n$ encoded in unary (the
  proof is similar to that of \LTLEBRP).
\end{proof}

